ProtoDUNE Photon Detection System

The Deep Underground Neutrino Experiment (DUNE) is a long-baseline neutrino oscillation experiment aiming to measure the oscillation parameters with an unprecedented precision that will allow determining the CP violation phase in the leptonic sector and the neutrino mass ordering. The Far Detector of DUNE will consist of four 17 kton liquid argon Time Projection Chambers (LAr-TPC). Inside a LAr-TPC, a Photon Detection System (PDS) is needed to detect the scintillation light produced by the interacting particles. The PDS signal provides the interaction time for non-beam events and improves the calorimetric reconstruction. To validate DUNE technology, two large-scale prototypes, of 750 ton of LAr each, have been constructed at CERN, ProtoDUNE-HD and ProtoDUNE-VD. The PDS of both prototypes is based on the XArapuca concept, a SiPM-based device that provides good detection efficiency covering large surfaces at a reasonable cost. This document presents the preliminary performance of the ProtoDUNE-HD Photon Detection System, which has taken data from April to November 2024.

==> 2_VD.tex <==
PD-VD PDS design


XArapucas
PMTs
Xenon doping
